CityFlowER: An Efficient and Realistic Traffic Simulator with Embedded Machine Learning Models

Traffic simulation is an essential tool for transportation infrastructure planning, intelligent traffic control policy learning, and traffic flow analysis. Its effectiveness relies heavily on the realism of the simulators used. Traditional traffic simulators, such as SUMO and CityFlow, are often limited by their reliance on rule-based models with hyperparameters that oversimplify driving behaviors, resulting in unrealistic simulations. To enhance realism, some simulators have provided Application Programming Interfaces (APIs) to interact with Machine Learning (ML) models, which learn from observed data and offer more sophisticated driving behavior models. However, this approach faces challenges in scalability and time efficiency as vehicle numbers increase. Addressing these limitations, we introduce CityFlowER, an advancement over the existing CityFlow simulator, designed for efficient and realistic city-wide traffic simulation. CityFlowER innovatively pre-embeds ML models within the simulator, eliminating the need for external API interactions and enabling faster data computation. This approach allows for a blend of rule-based and ML behavior models for individual vehicles, offering unparalleled flexibility and efficiency, particularly in large-scale simulations. We provide detailed comparisons with existing simulators, implementation insights, and comprehensive experiments to demonstrate CityFlowER's superiority in terms of realism, efficiency, and adaptability.

==> 3method.tex <==
\section{DESCRIPTION}

Since this work is built upon the existing work CityFlow, aiming at improving the realistic behavior modeling while keeping a similar simulating efficiency. Thus, we follow the same \texttt{Road Network} structure for fast intersection logic. For \texttt{Car Following Model} and \texttt{Lane Change Model}, we designed an embedded architecture to incorporate realistic learned models into the underlying simulator, and rebuild the simulator for consistent simulation support.


\subsection{System Design}
In CityFlow+, the realistic simulation relies on realistic behavior models, which are trained by behavior data using Imitation Learning (IL) or Behavior Cloning (BC) methods. The behavior data could either be collected from a more realistic simulator's rollout process or from real-world demonstrations. 

Once the system has access to trained behavior models, it will import the \texttt{Car\_following} or \texttt{Lane\_changeing} models in the simulation functions like \textit{get\_following\_speed} or \textit{get\_lane\_actions}. After that, the simulator will be rebuilt based on the new structure with imported behavior models. It is worth noting that, with the rebuilding process, all the public functions and APIs for the original CityFlow simulator will remain identical, which could seamlessly update to the existing projects.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/demo.pdf}
    \caption{The overview of the CityFlow+ for more realistic behavior modeling}
    \label{fig:levels}
\end{figure}


\subsection{Incorporate the Customizable Models}

The Python Interface is designed as below (\textcolor{red}{to be finished}):...

model requirement


\textcolor{red}{how to load the ML models into the simulator}

% \begin{center}
% \begin{minipage}{.95\textwidth}
% \label{lis:code}
% \begin{lstlisting}[language=Python,  label=code:api-example]
% def get_following_speed(params):
%     try:
%         result = Execution(target)
%     except Error as e:
%     print(e)
%     return result
            
% \end{lstlisting}
% \end{minipage}
% \end{center}



% \subsection{Front End}

